Efficient Exploration of the Rashomon Set of Rule Set Models

Today, as increasingly complex predictive models are developed, simple rule sets remain a crucial tool to obtain interpretable predictions and drive high-stakes decision making. However, a single rule set provides a partial representation of a learning task. An emerging paradigm in interpretable machine learning aims at exploring the Rashomon set of all models exhibiting near-optimal performance. Existing work on Rashomon-set exploration focuses on exhaustive search of the Rashomon set for particular classes of models, which can be a computationally challenging task. On the other hand, exhaustive enumeration leads to redundancy that often is not necessary, and a representative sample or an estimate of the size of the Rashomon set is sufficient for many applications. In this work, we propose, for the first time, efficient methods to explore the Rashomon set of rule set models with or without exhaustive search. Extensive experiments demonstrate the effectiveness of the proposed methods in a variety of scenarios.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> additional_baselines.tex <==
In order to offer a more complete assessment of the performance of the methods we propose, 
we compare \bb, \bbSTS and \algac against three simpler alternative approaches. 
Such simple alternative approaches are intended to serve as baselines to gain a deeper understanding of the advantages offered by \bb, \bbSTS and \algac. 
Next, the three simple baseline approaches are described in detail. 

\begin{itemize}
	\item  \naivebb: a naïve search algorithm which does not enforce any pruning of the search space. The \naivebb algorithm is analogous to \bb, but it exhaustively considers all rule sets and test them for inclusion into the Rashomon set. 
	
	\item  \cpsat: a constraint programming solver that uses SAT (satisfiability) methods. In particular, in order to leverage an highly optimized SAT solver, we encode the problem as follows. 
	
	A data record $\pr{\vx_n, y_n}$ is said to be positive if $y_n = 1$ and negative otherwise. 
	Let $\mathbf{N}_I$ be an indicator matrix such that $\mathbf{N}_{I_{i,j}} = 1$ if the $i$-th negative data record is covered by the $j$-th rule. Similarly, let $\mathbf{P}_I$ be an indicator matrix such that $\mathbf{P}_{I_{i,j}} = 1$ if the $i$-th positive data record is covered by the $j$-th rule. 
	Let $\nrules$ be the number of input rules. 
	Finally, let $|\ds|^-$ and $|\ds|^+$ denote the number of negative and positive data records, respectively. 
	
	We encode the counting problem as the problem of finding all $\textbf{x} \in \{0,1\}^M$,
	such that: 
	\begin{equation}\label{eq:sat1}
	 \frac{ z_{FP} }{N} + \frac{ z_{FN} }{N} + \lambda \sum_{j=1}^M \textbf{x}[j] \leq \ub,
	 \end{equation}
	where: 
	\begin{equation}\label{eq:sat2}
	z_{FP} = \sum_{i \in 1}^{|\ds|^-} \min (\mathbf{N}_{I_i}\textbf{x}, 1)
	\end{equation}
	and 
	\begin{equation}\label{eq:sat3}
	z_{FN} = \sum_{i \in 1}^{|\ds|^+} \max(1  - \mathbf{P}_{I_i}\textbf{x}, 0).
	\end{equation}
	Here, $\textbf{x}[j]$ is the $j$-th entry of $\textbf{x}$, $\mathbf{N}_{I_i}\textbf{x}$ denotes the dot product between the $i$-th row of $\mathbf{N}_I$ and the vector $\textbf{x}$.  Similarly, $\mathbf{P}_{I_i}\textbf{x}$ denotes the dot product between the $i$-th row of $\mathbf{P}_I$ and $\textbf{x}$. 
	As $\mathbf{N}_{I_i}$, $\mathbf{P}_{I_i}$ and $\textbf{x}$ are all binary vectors, the dot product corresponds to a set intersection. 
	
	Given the set of constraints described in Equations~\ref{eq:sat1},~\ref{eq:sat2} and~\ref{eq:sat3}, we find all rule sets by resorting to a state-of-the-art solver for constraint programming~\cite{cpsatlp}.
	
	
	\item \is: a method based on Monte Carlo simulation, where we simulate a large number of rule sets and evaluate the proportion of rule sets that belong to the Rashomon set. 
	The proportion can then be mapped to the corresponding count by multiplying by the total number of rule-set models, that can be easily computed.
	However, plain Monte Carlo sampling is extremely inefficient for very rare events~\cite{cerou2012sequential}.
	As suggested by~\citet{semenova2019study}, in order to estimate the size of the Rashomon set, it is preferable to use the Monte Carlo method known as importance sampling~\cite{tokdar2010importance}. 
	The main idea underlying importance sampling is to bias the sampling distribution in favour of the rare event, which, in our case, corresponds to the event that a rule set belongs to the Rashomon set. 
	In particular, we use the training data to devise a proposal sampling distribution biased towards the Rashomon set. 
	The importance sampler is then designed as follows. 
	
	
	\begin{itemize}
		\item Given the set of pre-mined rules \candrules, compute the reciprocal individual contribution of each rule $r$ to the loss, namely $\Delta \loss(r) = \frac{1}{\lossp(r) + \lossz(r)}$. 
		The penalty term for complexity is not included in $\Delta \loss(r)$ since each rule contributes equally to such penalty term. 
		
		\item Normalize $\Delta \loss(r)$ as $\Delta \loss'(r) = \frac{ \Delta \loss(r) } { \sum_{r' \in \candrules¸} \Delta \loss(r') }.$
		
		
		\item Sample $N_{rep}$ ($1,000,000$ by default) times an integer  $t$ uniformly at random in the interval $[ 1 , |\candrules| ]$ and a rule set $\rs$ of size $t$ with probability $p(d) = \Delta \loss'(r_1) \Delta \loss'(r_2) \dots \Delta \loss'(r_n).$ While $p(\cdot)$ neglects possible dependencies between the rules in $\rs$, it is effective in biasing the sampling towards the Rashomon set.  
		
		\item Compute the importance sampling estimate $\frac{1}{N} \sum_{i=1}^N f_I(\rs) \frac{u(\rs)}{p(\rs)} $ where $f_I(\rs)$ is an indicator function for the event that $\rs$  belongs to the Rashomon set, $p(\cdot)$ is the proposal distribution described above, and $u(\cdot)$ is the target distribution, i.e., the uniform distribution. 
		
		
		
		
		
		
		
	\end{itemize}
	In practice, to enhance the performance of \is,
	instead of sampling rule sets of length up to $|\candrules|$, we sample rule sets of length up to the upper bound obtained by setting $\rs = \emptyset$ in Theorem~\ref{theorem:number_of_rules_start}.
	
	
	Further, \is, unlike \cpsat and \naivebb, cannot be used to enumerate or sample near-uniform rule sets in the Rashomon set, but only to only to address the counting problem. 
	In Section~\ref{sec:experiment_results}, we show a comparison of the proposed methods against \naivebb, \cpsat and \is in a simple instance of the counting problem. 
	
	
\end{itemize}
















==> approx_algos.tex <==



\input{illustrations/cbb}

In this section, we consider the approximate version of the counting and sampling problems.
We leverage the approximation framework proposed by Meel~\cite{meel2017constrained}.


The approximate counting and sampling problems can be formalized as follows.
Consider any given of candidate rules $\cands$, objective function $\obj \pr{\cdot, \lambda}$, and objective upper bound $\ub \in \real^+$.

\spara{Approximate counting.}
We say a counting algorithm $\algc$ is \textit{an approximate counter} if
for some given tolerance parameter $\tol \in \real^+$, and confidence parameter $\confi \in \spr{0, 1}$, it is guaranteed that

\begin{equation}
  \label{}
  \proba{\frac{\abs{\rssshort}}{1+\tol} \le \algc(\cands, \obj, \tol, \confi) \le  \pr{1+\tol}  \cdot \abs{\rssshort}} \ge 1 - \confi,
\end{equation}

where we drop the dependence on $\ub$ and $\lambda$ for brevity.

\spara{Almost uniform sampling.}
We say a sampling algorithm $\algs$ is \textit{an almost-uniform sampler} if
for some given tolerance parameter $\tol \in \real^+$ and for any $d \in \rssshort$, it is guaranteed that

\begin{equation}
  \label{}
  \frac{1}{1+\tol}\le  \proba{\algs \pr{\cands, \obj, \ub, \tol} = d} \le  (1+\tol)
\end{equation}

\subsection{A random partitioning-based framework}

\cite{meel2017constrained} proposes two meta algorithms for the above problems which enjoys strong probabilistic guarantee.
The framework relies on an enumeration oracle, which is assumed to be SAT solver-based in their work.
We propose to implement the oracle using an adhoc branch-and-bound algorithm, which enables better scalability.

In the sequel, we first describe Meel's algorithmic framework and then propose our implementation of the oracle.%

\spara{The approximate counting algorithm}.
The counting algorithm (described in Algorithm~\ref{alg:approxcount}) uses randomly generated parity constraints
to partition the solution space into ``small'' cells,
where finding the right parameters to get the desired cell sizes requires an iterative search (described in Algorithm~\ref{alg:logsearch}
).
The algorithm then invokes an oracle $\algbs$ to exactly measure the size of a random cell and uses as an estimate of $\abs{\rss(\cands)}$ given by the cell size multiplied by the number of cells.
Finally, The estimation is repeated on sufficiently many random cells (to achieve the desired confidence) and the median is returned.


\begin{proposition}[~\cite{meel2017constrained}]
  $\algac$ is an approximate counter for the Rashomon set counting problem.
\end{proposition}


\begin{algorithm}
  \caption{\algac\xspace takes in an instance of decision set learning and outputs an estimate of the Rashomon set size}
  \label{alg:approxcount}  
  \begin{algorithmic}  
    \STATE $\budget \define 1+ 9.84 \pr{1 + \frac{\tol}{1+\tol}}^2$
    \STATE $\solset \define \algbs \pr{\instance, \budget}$
    \IF{$\abs{\solset} < \budget$}  
    \STATE \Return {$\abs{\solset}$}
    \ENDIF
    \STATE $t \define \ceil{17 \log_2 \pr{3 / \confi}}$
    \STATE $\ncells  \define 2;\ C \define \spr{};\ i \define 0$
    \WHILE{$i < t$}
    \STATE increment $i$
    \STATE$\pr{\ncells, \solcount} \define \algacc \pr{\instance, \budget, \ncells}$
    \STATE add $\solcount$ to $C$ if $\ncells \neq \nullresult$
    \ENDWHILE
    \STATE \Return $\text{median}\pr{C}$
    \end{algorithmic}    
\end{algorithm}

\begin{algorithm}[tb]
  \caption{\algacc\xspace takes in one instance of decision set learning and outputs the number of cells and an estimate of $\abs{\rss}$.}
  \begin{algorithmic}
    \STATE Draw $\mA$ from $\bindom^{\abs{\cands} \times \pr{\abs{\cands} - 1}}$ uniformly at random
    \STATE Draw $\vb$ from $\bindom^{\abs{\cands} - 1}$ uniformly at random
    \STATE $\solset \define \algbs \pr{\instance, \mA, \vb, \budget, \prevncells}$
    \IF{$\abs{\sols} \ge \budget$}    
    \STATE  \Return{\nullresult}
    \ENDIF
    \STATE $\pr{m, c} \define \algls \pr{\instance, \Axb, \budget, m}$
    \STATE \Return{$\pr{2^m, c \times 2^m}$}
  \end{algorithmic}
\end{algorithm}

\cnote[Han]{Explain what $\algls$ does, e.g., what does the value of $\bigcell$ mean}
\cnote[Han]{why $\prevm$ is not updated?}

\begin{algorithm}
  \caption{\algls\xspace finds the number of constraints under which the number of feasible solutions is below but closest to $\budget$.}
  \label{alg:logsearch}
  \begin{algorithmic}
    \STATE $\loidx \define 0;\ \hiidx \define \abs{\cands} - 1; \ m \define \prevncells$
    \STATE $\bigcell[0] \define 1;\ \bigcell[\abs{\cands} - 1] \define 0; \ \bigcell[i] \define \nullresult\; \forall i \not\in \set{0, \abs{\cands} - 1}$
    \WHILE{\true}    
        \STATE $\solset \define \algbs \pr{\instance, \mA_{:m}, \vb_{:m}, \budget}$
        \IF{$\abs{\solset} \ge \budget$}
            \IF{$\bigcell \pr{m+1} = 0$}
                \STATE\Return{$m+1$}
            \ENDIF
            \STATE $\bigcell[i] \define 1\; \forall i \in \set{1, \ldots, m}$
            \STATE $\loidx \define m$
            \IF{$|m - \prevm| < 3$}
                \STATE $m \define m+1$
            \ELSIF{$2 \cdot m < \abs{\cands}$}
                \STATE $m \define 2 \cdot m$
            \ELSE
                \STATE $m \define \pr{\hiidx + m} / 2$
            \ENDIF  
        \ELSE
            \IF{$\bigcell[m-1] = 1$}
                \STATE\Return{$m$}
            \ENDIF
            \STATE $\bigcell \spr{i} \define 0\; \forall i \in \set{m, \ldots, \abs{\cands}}$
            \STATE $\hiidx \define m$
            \IF{$|m - \prevm| < 3$}
                \STATE $m \define m -1$
            \ELSE
                \STATE $m \define (m + \loidx) / 2$
            \ENDIF
        \ENDIF
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}


\spara{Approximate uniform sampling}.
The sampling algorithm builds upon the techniques for approximate counting -- the solution space is randomly partitioned into cells of the ``right'' size and samples are drawn uniformly random from a randomly selected cell.

\begin{algorithm}[tb]
  \caption{\algsample draws a random sample from $\rss$ almost uniformly at random}
  \begin{algorithmic}[1]
      \STATE $\pr{\kappa, \unigenpivot} \define \algkappapivot(\tol)$
      \STATE $\hibudget \define 1 + (1 + \kappa) \unigenpivot$
      \STATE $\lobudget \define \frac{1}{1 + \kappa} \unigenpivot$
      \STATE $\solset  \define \algbs(\instance, \hibudget)$
      \IF{$\abs{\solset} \le \lobudget$}
          \STATE \Return{$s \sim \unirandom \pr{\solset}$}
      \Else
          \STATE $\solcount \define \algac(\instance, 0.8, 0.8)$
          \STATE $q \define \ceil{\log\solcount + \log 1.8 - \log \unigenpivot}$
          \STATE $i \define q - 4$
          \STATE $\mA \sim \unirandom \pr{\bindom^{\abs{\cands} \times \pr{\abs{\cands} - 1}}}$ and $\vb \sim \unirandom \pr{\bindom^{\abs{\cands} - 1}}$
          \REPEAT
              \STATE $i \define i + 1$
              \STATE $\solset \define \algbs \pr{\instance, \mA_{:i} x = \vb_{:i}, \hibudget}$
          \UNTIL{$\lobudget \le \abs{\solset} \le \hibudget$ or $i = q$}
          \IF{$ \lobudget \le \abs{\solset} \le  \hibudget$}
              \STATE \Return{$\unirandom \pr{\solset}$}
          \ELSE
              \STATE \Return $\nullresult$
          \ENDIF
      \ENDIF
  \end{algorithmic}
\end{algorithm}

\begin{proposition}[~\cite{meel2017constrained}]
  \algsample is an almost-uniform sampler \inote{to what problem?}
\end{proposition}


\subsection{Parity-constrained enumeration}
\label{subsec:label}


\begin{problem}[\textbf{Budgeted enumeration with parity constraints}]
  \label{prob:budgeted-enum}
  Given a set of decision rule candidates $S$, objective function $\loss$, objective upper bound  $\ub$, a parity constraint system characterized by $\Axb$ and an integer $B$, find at most $B$ decision sets s.t.
  \begin{itemize}
  \item $\obj \pr{d} \le \ub$
  \item $\Axb$
  \end{itemize}  
\end{problem}


\cnote[Han]{Maybe we can assume that $\Axb$ is in its reduced row echelon form (since it is equivalent to the original form), to simplify the notations a bit.} %
For a given a linear system $\Axb$, we consider the matrix to be in its reduced row echelon form and the resulting system becomes $\Axbr$.
Since for any $x$, $\Axbr \iff \Axb$, replacing the constraint $\Axb$ in Problem~\ref{prob:budgeted-enum} with $\Axbr$ results in a problem with the same set of feasible solutions.
\inote{Is still it true if rows are swapped? But it does not matter for the counting and sampling algorithm}.
\inote{I guess so, the RREF is unique for a given row space (the order of the vector in the row space basis is irrelevant.. - MC)}.


Further, matrices in their reduced row echelon form have some important properties revealed, such as their ranks and pivot positions.
These properties turn out to be essential for the algorithm development.
Therefore, we assume $\Axb$ is in its reduced row echelon form in the sequel.

Then for a matrix $\mA$, we use $\pivotA$ to denote its pivot table, where $\pivotA \spr{i}$ is the column index of the pivot position in the $i$th row, for any $i\in\spr{\rank \pr{\mA}}$.
In addition, we denote $\pvtsetA = \set{\pivotA[i] \mid i \in \rank(\mA)}$ and $\freesetA = \set{0, \ldots, \nrules-1} \setminus \pvtsetA$, i.e., the pivot column indices and free column indices in $\mA$, respectively.
When context is clear, we drop the subscript $\mA$ and use $\pivot[i]$, $\pvtset$, and $\freeset$ for brevity.

We then correspond the rules with the pivot positions in $\mA$.
We call the $j$th rule a \textit{pivot rule} if the $j$th column in $\mA$ corresponds to some pivot position, i.e., $\exists i \in \spr{\rankA} \text{ s.t. } \pivot \spr{i} = j$. Otherwise, the rule is called a \textit{free rule}.

For a given prefix $d$, we denote $\pvtset(d) = \pvtset \cap d$, i.e., the set of pivot rules in $d$ and $\freeset(d) = \freeset \cap d$, i.e., the set of free rules in $d$.

In the following branch and bound algorithms, we only check the addition of free rules and the selection of free rules will determine the selection of the pivot rules, according to $\Axb$.




\cnote[Han]{when context is clear, we can drop the subscript $A$, e.g., $\pivotA[i] \rightarrow \pivot[i]$}
\subsection{A naive branch-and-bound algorithm}

\subsubsection{Description}
\label{subsec:label}


We propose a branch-and-bound algorithm, which builds upon a technique for enumerating solutions to a linear system $\Axb$ in finite field 2.
During the enumeration process, solutions are pruned on the fly to satisfy $\obj(d) \le \ub$

\spara{Enumerating feasible solutions to $\Axb$.}
For the sake of exposition, we first consider the problem of enumeration solutions to $\Axb$ and then add the constraint $\obj(d) \le \ub$ on top.
A straight-forward way to enumerate all feasible solutions to $\Axb$ is by converting the linear system to its reduced row echelon form, identifying the pivot and free variables, and considering all possible assignments of the free variables (and the pivot variables are assigned accordingly).

A toy example consisting of 3 constraints and 5 variables is given below:
on the left shows the original $\Axb$
and on the right its reduced row echelon form,
where the pivot columns ($x_1$, $x_2$, and $x_4$) are highlighted in bold.


\[
\begin{bmatrix}
 1 & 1 & 1 & 1 & 1 \\
 0 & 1 & 1 & 1 & 1 \\
 0 & 0 & 0 & 1 & 1 \\
\end{bmatrix}
\begin{bmatrix}
  x_1\\
  x_2\\
  x_3\\
  x_4 \\
  x_5
\end{bmatrix}
=
\begin{bmatrix}
 0 \\
 1 \\
 1 \\
\end{bmatrix}
\rightarrow
\begin{bmatrix}
  \mbold{1} & \mbold{0} & 0 & \mbold{0} & 0 \\
  \mbold{0} & \mbold{1} & 1 & \mbold{0} & 0 \\
  \mbold{0} & \mbold{0} & 0 & \mbold{1} & 1 \\
\end{bmatrix}
\begin{bmatrix}
  x_1\\
  x_2\\
  x_3\\
  x_4 \\
  x_5
\end{bmatrix}
=
\begin{bmatrix}
 1 \\
 0 \\
 1 \\
\end{bmatrix}
\]

From the reduced row echelon form,
the set of feasible solutions can be characterized by $x_1  = 1, x_2  = x_3 , x_4  = 1+ x_5$\footnote{Note that $x=-x$ in finite field 2}. 
Or equivalently,

\[
  x =
  \begin{bmatrix}
    x_1\\
    x_2\\
    x_3\\
    x_4 \\
    x_5
  \end{bmatrix}
  =
  \begin{bmatrix}
    1\\0\\0\\1\\0
  \end{bmatrix}
  +
  \begin{bmatrix}
    0\\1\\1\\0\\0
  \end{bmatrix}
  x_3
  +
  \begin{bmatrix}
    0\\0\\0\\1\\1
  \end{bmatrix}
  x_5
\]



In other words, the feasible solutions can be enumerated by substituting $[x_3, x_5] \in \set{0, 1}^2$ in the above equation.



To integrate the above idea into the branch-and-bound algorithm, we need to make 4 changes on top of Algorithm~\ref{alg:noninc-bb}.

\begin{enumerate}
\item In the inner loop, instead of checking all rules, we check only the rules corresponding to the free columns. For instance, in the above example, only $x_3$ and $x_5$ are checked.
\item {
    While adding a rule $j$ to a given prefix, we need to check if the satisfiability of some of the parity constraints can be determined already.
    And if so, add the relevant pivot rules to make sure these constraints are satisfied.
    This change is implemented by the function $\ensurenoviolation$.
  }
\item {When checking the objective lower bound, the pivot rules added by $\ensurenoviolation$ should be considered}
\item When trying to yield a solution, we need to guarantee all parity constraints are satisfied. This requirement is fulfilled by the function $\ensuresatisfaction$.
\item {Finally, the algorithm terminates when either $\budget$ solutions are found or all feasible solutions are found}
\end{enumerate}

\cnote[Han]{maybe refer the change to the line in the algorithm}


To implement the second change, we need to add pivot rules to a given prefix to ensure the solution does not violate $\Axb$.

Given a prefix $d$ and a constraint $\mA_i x = \vb_i$, we say the satisfiability of $\mA_i x = \vb_i$ is \textit{determined} by $d$ if $\dmax \ge \btbl[i]$.
In other words, adding any rule above $\dmax$ does not affect the satisfiability of $\mA_i x = \vb_i$.
For instance in the above example, the satisfiability of $x_2 + x_3 = 1$ is determined by $\set{1, 4}$ and $\set{4}$ but not by $\set{1}$.

We use an integer array called \textit{boundary table} to check if the satisfiability of constraints in $\Axb$ can be determined by a given prefix.
The boundary table of a matrix $\mA$ is denoted as $\btblA: \spr{\rankA} \rightarrow \spr{\nrules}$, which maps a row index to a column index. 
For any $i \in \spr{\rankA}$, $\btblA \spr{i} = \max \set{j \mid \mA \spr{i, j} = 1 \text{ and } j \neq \pivotA \spr{i}}$ if $\sum_j \mA \spr{i, j}> 1$ , otherwise $\btbl \spr{i} = -1$.
In other words, $\btblA \spr{i}$ is the largest non-zero non-pivot column index of $\mA_i$ if it exists, otherwise it is $-1$.
For instance, the boundary table of the above example is $\btbl=\spr{-1, 2, 4}$.

Given a prefix $d$, we say $d$ is \textit{non-violating} if the constraints in $\Axb$ that are determined by $d$ are all satisfied.
For instance, $\set{1, 4}$ and $\set{1}$ are non-violating, while $\set{4}$ is not (it determines $x_1 = 1$ but violates it).
Further, we say $d$ is \textit{minimally non-violating} if
$(i)$ $d$ is non-violating
and $(ii)$ removing any rule $\pvtset(d)$ from $d$ violates some constraint no matter which subset of $\set{\freeset(d)_{max}, \ldots, \nrules}$ is added to $d$.
For instance, $d=\set{1, 2, 3}$ in the above example is minimally non-violating because removing either $2$ or $3$ violates $x_2 + x_3 = 0$ or $x_1=1$, no matter which subset of $\set{4, 5}$ is added.

We rely on the notion of minimal non-violation to determine a minimal set of pivot rules required to be added to a prefix $d$ in order for $d$ to be non-violating.
Such notion ensures that no redundant pivot rules are added, thus the proposed branch-and-bound algorithm does not falsely prune away prefixes.

Last, for a minimal non-violating prefix $d=\pvtset (d) \cup \freeset (d)$, we call each pivot rule $k \in \freeset (d)$ a \textit{necessary pivot} for $\freeset(d)$.

\bigskip

Next we extend the hierarchical objective lower bound to account for the parity constraint.

\begin{theorem}[\textbf{Extended hierarchical objective lower bound}]
  Let $d$ be a prefix with free rules only, let $e$ be the set of necessary pivot associated with $d$, in other words $d \cup e$ is minimally non-violating.
  For any prefix $d'$ that starts with $d$, denote $e'$ as the set of necessary pivots for $d'$, 
  it follows that $\lb(d \cup e) \le  \obj(d' \cup e')$
\end{theorem}
\begin{proof}
  We first show $e \subset e'$.

  Consider each $p \in e$, since $p$ is a necessary pivot for $d$, there must exist some constraint $\mA_i x = \vb_i$ s.t. $\mA_i \xd \neq \vb_i$ and $d$ determines the satisfiability of it.
  Since $d \subset d'$, the constraint is also determined by $d'$ because $\dpmax > \dmax \ge \btbl[i]$.
  Further since $d'$ starts with $d$, no rules below $\dmax$ are in $d'$, thus $\mA_i \xd \neq \vb_i$ holds.
  Therefore, $p$ is a necessary pivot for $d'$.

  In other words, $\abs{d \cup e} \le \abs{d' \cup e'}$.

    \medskip
  
    Next the proof of $\lossp (d' \cup e') \ge \lossp(d \cup e)$ is straight-forward.
    We need to re-order the rules in $d \cup e$ and $d' \cup e'$ such that  $d' \cup e'$ starts with $d \cup e$.
    Then Theorem~\ref{thm:hier-obj-lb} implies $\lossp (d' \cup e') \ge \lossp(d \cup e)$, which concludes the proof.
\end{proof}  

To generalize, consider a sequence of prefixes $\spr{d_1, \ldots, d_N}$ such that each prefix $d_i$ consists of free rules only and starts with all previous prefixes in the sequence.
Then consider the corresponding sequence of extended prefixes $\spr{d_1 \cup e_1, \ldots, d_N \cup e_N}$, where $e_i$ is the set of necessary pivots associated with $d_i$.
It follows that the corresponding sequence of objective lower bounds $b(d_i \cup e_i)$ increases monotonically with $i$.
This is precisely the structure required and exploited by the branch-and-bound algorithm illustrated in Algorithm~\ref{alg:noninc-cbb}.


\begin{algorithm}[tb]
  \caption{Naive branch and bound to solve Problem~\ref{prob:budgeted-enum}.
    The incremental calculation of objective lower bound and objective value is omitted for brevity.}
  \label{alg:noninc-cbb}
  \begin{algorithmic}    
    \STATE $\mA, \vb \define \rref \pr{\mA, \vb}$
    \IF{$\Axb$ is unsolvable}
        \STATE {exit}
    \ENDIF
    
    \STATE $\solcounter \define 0$
    \STATE $d_s \define \ensuresatisfaction\pr{\emptyset, \mA, \vb}$
    \IF{$R(d_s) \le \ub$}    
        \STATE increment $n$ and yield $d_s$
    \ENDIF
    \STATE $d_q \define \ensurenoviolation\pr{\emptyset, \mA, \vb}$
    \STATE $Q \define \queue\pr{\pr{d_q}}$
    \WHILE{$Q$ is not empty and $\solcounter < B$}
        \STATE $d \define Q.pop()$
        \FOR{$j = \pr{\freeset(d)_{max} + 1}, \ldots, M \text{ and } j \text{ is free}$}    
            \STATE $d' \define d \cup \set{j}$
            \IF{$b(d') \le \ub$}
                \STATE $\pvtextone \define \ensurenoviolation\pr{d', \mA, \vb}$
                \IF{$b(d' \cup \pvtextone) < \ub$}        
                    \STATE$Q.\text{push}(d')$
                \ENDIF
                \STATE $\pvtexttwo \define \ensuresatisfaction\pr{d', \mA, \vb}$
                \STATE $d_s \define d' \cup \pvtexttwo$
                \IF{$R(d_s) \le \ub$}
                    \STATE increment $\solcounter$ and yield $d_s$
                \ENDIF
            \ENDIF
        \ENDFOR
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}


\bigskip

\subsubsection{Ensuring minimal non-violation}

The procedure $\ensurenoviolation$ (described in Algorithm~\ref{alg:ensure-non-vio}) checks if each constraint can be determined by the given prefix $d$. If yes and the constraint is not satisfied by $d$, the corresponding pivot rule is added to ensure satisfaction.

We show that $\ensurenoviolation$ indeed produces minimally non-violating prefixes.

\begin{theorem}
  For any prefix $d$ with free rules only, $\ensurenoviolation(d, \cdot)$ returns a set of pivot rules $e$ such that $d \cup e$ is minimally non-violating, in other words, $e$ is all the necessary pivots for $d$.
\end{theorem}




\begin{algorithm}[tb]
  \caption{
    $\ensurenoviolation$ extends a prefix $d$ by a set of necessary pivot rules such that the new prefix is minimally non-violating
  }
  \label{alg:ensure-non-vio}
  \begin{algorithmic}
    \STATE $\vr = \vb - \mA \cdot \xd$
    \STATE $\pvtext \define \emptyset$    
    \FOR{ $i = 1, \ldots, \rank\pr{\mA}$ }
        \IF{$\vr[i] = 1$ and $\dmax \ge \btbl[i]$}
            \STATE $\pvtext \define \pvtext \cup \pivotA[i]$
        \ENDIF
    \ENDFOR
    \STATE \Return{$\pvtext$}
  \end{algorithmic}

\end{algorithm}


The proof consists of two parts.

\begin{lemma}
  For any prefix $d$ with free rules only, all pivots returned by $\ensurenoviolation(d)$ are necessary for $d$
\end{lemma}
\begin{proof}
  We consider each $i \in\spr{\rankA}$ that has $\pivot \spr{i}$ added.
  First, since $\vr_i = \vb_i - \mA_i \cdot \xd = 1$, some rule $j$ s.t. $\mA_{i, j}=1$ must be added to ensure $\vb_i = \mA_i \cdot x$.
  Second, since $\dmax \ge \btblA[i]$, there are no free rules larger than $\dmax$ that can be added to ensure $\vb_i = \mA_i \cdot x$.
  In other words, the rule $\pivot[i]$ must be added, making it necessary for $d$.
\end{proof}

\begin{lemma}
  For any prefix $d$ with free rules only, no other necessary pivots for $d$ are absent in $\ensurenoviolation(d)$
\end{lemma}
\begin{proof}
  We prove by contradiction.  
  Suppose there exists some $i \in\spr{\rank\pr{\mA}}$ such that $i$ is necessary for $d$ but $\pivot \spr{i}$ is not added.
  That $i$ being necessary for $d$ implies $\vb_i \neq \mA_i \cdot \xd$.
  Further, $\pivot \spr{i}$ being excluded implies some free rule $j$ must be added to ensure $\vb_i = \mA_i \cdot x$.
  Because any free rule $j < \dmax$ cannot be added by algorithm construction, we must add some free rule $j > \dmax$ with $\mA_{i, j}=1$, which contradicts with $\dmax \ge \btblA[i]$.
\end{proof}








\subsubsection{Ensuring solutions' satisfiability}
Finally, when trying to yield a feasible prefix $d$, we need to make sure that $d$ indeed satisfies $\Axb$.
The satisfaction is guaranteed by the procedure $\ensuresatisfaction$ (described in Algorithm~\ref{alg:ensure-sts}).

\begin{algorithm}[tb]
  \caption{
    $\ensuresatisfaction$ adds a set of pivot rules to the prefix $d$ so that $\Axb$ is satisfied.
  }
  \label{alg:ensure-sts}
  \begin{algorithmic}
    \STATE $\vr = \vb - \mA \cdot \xd$
    \STATE $\pvtext \define \emptyset$
    \FOR{ $i = 1, \ldots, \rank\pr{\mA}$ }
        \IF{$\vr[i] = 1$}
            \STATE $\pvtext \define \pvtext \cup \pivotA[i]$
        \ENDIF
    \ENDFOR
    \Return{$\pvtext$}
  \end{algorithmic}
\end{algorithm}

The correctness is straight-forward.

\begin{theorem}
  For any prefix $d$ with free rules only, let $\pvtext$ be the set of pivots returned by $\ensuresatisfaction(d)$, it follows that $\mA x_{d \cup \pvtext} = \vb$.
\end{theorem}
\begin{proof}
  If for some $i$, $\mA_i \xd = \vb$, the algorithm does not add $\pivot\spr{i}$, maintaining the equality.
  If $\mA_i \xd \neq \vb$, $\pivot\spr{i}$ is added, making equality holds.
  \cnote[Han]{The result looks obvious. Is using theorem an overkill?}
  \cnote[MC]{ I think it is fine, if it cannot be presented as a lemma for the main result stating that the algorithm is correct. Alternatively, we could present this as "proposition". }
\end{proof}


\subsection{Incremental computation}
\label{subsec:label}

\cnote[Han]{To think about: can we simplify the proofs?}
Pp
To enable incremental computation, we need a few data structures.

For a given prefix $d$, we denote $\vz \in \bindom^{\ncons}$ as its \textit{parity states vector}, where $\vz \spr{i} = \mA \xd - \vb$ for any $i\in\spr{\ncons}$.
If $d = \emptyset$, $\vz = \vzero$.

For any $i \in \spr{\ncons}$ and any prefix $d$ such that $\mA_i \xd = \vb_i$, we say the satisfiability of the $i$th constraint is \textit{guaranteed} if adding any set of rules whose index is above $\dmax$ cannot make $\mA_i \xd \neq \vb_i$. 
It is easy to show that the satisfiability of the $i$th constraint is guaranteed by a prefix $d$ if $\mA_i \xd = \vb_i$ and $\dmax \ge \btbl[i]$. The second condition ensures no rules above $\dmax$ can affect the satisfiability of the $i$th constraint.

In the proposed algorithm, we use \textit{a satisfiability vector} $\vs \in \bindom^{\ncons}$  to track if the constraints are guaranteed or not, where $\vs[i] = 1$ indicates the $i$th constraint is guaranteed and $\vs[i]=0$ otherwise.
If $d = \emptyset$, $\vs = \vzero$.


\bigskip
In the queue data structure, each item contains: $d'$, the prefix to be checked later, $b(d')$, its lower bound, $\vu'$, the uncaptured vector, two other vectors $\vs'$ and $\vz'$.

We maintain a few invariants on the queue items: for each prefix $d'$ and its associated vectors $\vs'$ and $\vz'$,, 

\begin{enumerate}
\item $\vs'$ is the corresponding satisfiability vector of $d'$
\item $\vz'$ is the corresponding parity states vector of $d'$
\item $d'$ contains all necessary pivot rules for $\freeset \pr{d'}$
\end{enumerate}

Next we show that the invariants are maintained by Algorithm~\ref{alg:inc-ensure-no-violation}.




\cnote[Han]{The proof looks like an explanation to me. Is a proof really needed?}
\begin{theorem}
  For a given prefix $d' = d \cup \set{j}$, where $j > \dmax$,
  let $\vs$ and $\vz$ be the corresponding satisfiability vector and parity state vector of $d$, respectively,.
  Denote the vectors returned by $\incensurenoviolation \pr{j, \vz, \vs, \mA, \vb}$ as $\vs'$ and $\vz'$.
  It follows that $\vs'$ and $\vz'$ are the corresponding satisfiability vector and parity state vector of $d'$, respectively.
\end{theorem}

\begin{proof}


  For every $i\in \spr{\rankA}$, there are two cases when the procedure does not need to do anything.
  (1) if $\vs[i] = 1$,  satisfiability of the $i$th constraint is guaranteed by $d$ already.
  (2) if $\mA[i, j] = 0$, rule $j$ does not affect the satisfiability of the $i$th constraint

  If the above conditions are not met, i.e.,  $\mA[i, j] = 1$ and $\vs[i] = 0$,
  There are 2 cases to consider:
  
  (1) If $j = \btblA[i]$, the satisfiability of the constraint can be guaranteed by two sub-cases:
  
  \indent\indent (1.1) if $\vz'[i] = \vb[i]$, we need to add $\pivot[i]$ to $d$ to maintain $\vz'[i] = \vb[i]$ and $\vz'[i]$ stays unchanged.
  
  \indent\indent (1.2) if $\vz'[i] \neq \vb[i]$, no other rule is added besides $j$ and $\vz'[i]$ is flipped to ensure $\vz'[i] = \vb[i]$.

  (2) If $j < \btblA[i]$, the satisfiability of the constraint cannot be guaranteed. No pivot rules are added and we simply flip $\vz'[i]$.
  
\end{proof}


\begin{theorem}
  For a given prefix $d' = d \cup \set{j}$, where $j > \dmax$,
  let $\vz$ and $\vs$ be the parity state vector and satisfiability vector of $d$, respectively.
  Denote $e$ as the pivot set returned by $\incensurenoviolation(j, \vz, \vs, \cdot)$,
  it follows that $e \cup \pvtset \pr{d}$ are all the necessary pivots for $\freeset \pr{d'}$
\end{theorem}
We prove the above by induction.
Assuming $\pvtset \pr{d}$ are all necessary pivots for $\freeset \pr{d}$,
we show 1) $e$ are necessary $\freeset \pr{d'}$ and
2) no other necessary pivots are excluded from $e$
The two results are formalized below.

\begin{lemma}
  For a given prefix $d' = d \cup \set{j}$, where $j > \dmax$,
  let $\vz$ and $\vs$ be the parity state vector and satisfiability vector of $d$, respectively.
  Denote $e$ as the pivot set returned by $\incensurenoviolation(j, \vz, \vs, \mA, \vb)$,
  it follows that all pivot rules in $e$ are necessary for $\freeset\pr{d'}$.
\end{lemma}
\begin{proof}
  We only check the cases $i \in\spr{\rankA}$ such that $\vs[i] = 0$ and $\mA[i, j] = 1$, since only in this case the algorithm may add pivots.
  If $\vz'[i] = \vb[i]$, then adding the rule $j$ flips $\vz'[i]$ and make $\vz' \neq \vb$.
  To ensure $\vz'[i] = \vb$, some rule $j'$ s.t. $\mA_{i, j'}=1$ must be added.
  Since $j = \btblA[i]$, no free rules larger than $\dmax$ can be added to ensure $\vb_i = \vz'[i]$.
  In other words, the rule $\pivot[i]$ must be added, making it necessary for $d$.
\end{proof}



\begin{lemma}
  For a given prefix $d' = d \cup \set{j}$, where $j > \dmax$,
  let $\vz$ and $\vs$ be the parity state vector and satisfiability vector of $d$,
  and $\pvtext$ be the set of indices returned by $\incensurenoviolation(j, \vz, \vs, \mA, \vb)$, 
  it follows that $\pvtset(d') \cup e$ are all the  necessary pivots for $\freeset\pr{d'}$.
\end{lemma}
\begin{proof}
  We prove by induction.

  \textbf{Induction step.}
  Assume that $\pvtset \pr{d}$ are all the necessary pivots for $\freeset\pr{d}$.
  Then we prove by contradiction.
  Suppose that there exists some $i \in\spr{\rank\pr{\mA}}$ such that $\vs[i]=0$ and $\pivot[i]$ is necessary for $d'$ but $\pivot \spr{i} \not\in \pvtext$.
  That $\pivot[i]$ being necessary for $d'$ implies $\dpmax = j = \btbl[i]$  and $\vb_i \neq \mA_i \cdot x_{\free\pr{d'}}$.
  And $\pivot \spr{i} \not\in \pvtext$ implies some free rule $k$ must be added to ensure the equality.
  Because any free rule $k < j$ cannot be added by algorithm construction, we must add some free rule $k > j$ with $\mA_{i, j}=1$, implying $\dpmax > j = \btbl[i]$, which contradicts with $\dpmax = \btbl[i]$.

  \textbf{Basis step.} In this case, $d' = \emptyset$, i.e., $j=-1, d=\emptyset, \text{ with }\vs=\vz=\vzero$. Assume there exists some necessary pivot for $\emptyset$ s.t. $\pivot[i] \not\in \pvtext$, by line \inote{add reference to some line} in, it is either because $\vb[i] = 0$ or $\btblA[i] \ge 0$:
  1) $\vz[i] = \vb[i] = 0$ implies $\pivot[i]$ can be excluded from $\pvtext$, which contradicts with $\pivot[i]$ being necessary for $\emptyset$.
  2) $\btblA[i] \ge 0$ implies some free rule can be added to make $\mA_i x = \vb[i]$ hold, contradicting $\pivot[i]$ being necessary for $\emptyset$.
\end{proof}


Finally, we show the $\incensuresatisfaction$ ensures the extended solution satisfies $\Axb$.

\begin{theorem}
  For a given prefix $d' = d \cup \set{j}$, where $j > \dmax$,
  let $\vz$ and $\vs$ be the parity state vector and satisfiability vector of $d$,
  and $\pvtext$ be the set of pivots returned by $\incensuresatisfaction(j, \vz, \vs, \mA, \vb)$, 
  it follows that $d' \cup e$ satisfies $\Axb$
\end{theorem}
\begin{proof}
  If $d'=\emptyset$, i.e., $j=-1$, $\vs = \vz = \vzero$, then
  for every $i \in \rankA$, $\pivot[i]$ is added to $\pvtext$ only if $\vz[i] \neq \vb[i] = 1$.

  Otherwise, if $\vs[i]=1$, the constraint is satisfied already and the algorithm does nothing.
  If $\vs[i]=0$, meaning the constraint is not satisfied yet.

  There are two sub-cases:
  
\indent (1) The $j$th rule is relevant to the constraint, i.e., $\mA[i, j]=1$.
    Rule $\pivot[i]$ should be added to $\pvtext$ if $\vz[i] = \vb[i]$ since adding $\pivot[i]$ and $j$ flips $\vb[i]$ twice, maintaining $\vz[i] = \vb[i]$.

\indent (2) The $j$th rule is irrelevant to the constraint, i.e., $\mA[i, j]=0$.
    Rule $\pivot[i]$ should be excluded from $\pvtext$ if $\vz[i] \neq \vb[i]$ since adding $j$ alone flips $\vb[i]$, making $\vz[i] = \vb[i]$.
\end{proof}


\cnote[Han]{the psuedo-code is updated, update the proofs as well}

\begin{algorithm}[tb]
  \caption{
    $\incensurenoviolation$ considers adding rule $j$ to a given prefix (represented by $\vps$ and $\vsat$) and adds an additional set of necessary pivot rules to ensure that the new prefix does not violate $\Axb$. 
    The parity state vector and parity target vector are updated accordingly.
  }
  \label{alg:inc-ensure-no-violation}
  \begin{algorithmic}
    \STATE $\pvtext \define \text{an empty set}$
    \STATE $\vps' \define \text{copy}\pr{\vps}$, $\vsat' \define \text{copy}\pr{\vsat}$    
    \FOR{
      $i=1, \ldots, \rank \pr{\mA}$
    }
    \IF{$j=-1$}
        \IF{$\btblA[i]=j$}
          \STATE $\vs'[i] \define 1$
          \IF{$\vb[i]=1$}
              \STATE $\pvtext \define \pvtext \cup \set{\pivotA \spr{i}}$
              \STATE flip $\vps'[i]$
          \ENDIF
        \ENDIF
        \STATE \Continue
    \ENDIF
    
    \IF{ $\vsat' \spr{i} = 0$}
        \IF{$j \ge \btblA \spr{i}$}
          \STATE $\vsat' \spr{i} = 1$        
          \IF{$\mA\spr{i,j} = 1$}
            \IF{$\vps'\spr{i}=\vb\spr{i}$}{
              \STATE $\pvtext \define \pvtext \cup \set{\pivotA \spr{i}}$
            }
            \ELSE
              \STATE flip $\vps'[i]$
            \ENDIF            
          \ELSIF{$\vps'\spr{i} \neq \vb\spr{i}$}
              \STATE $\pvtext \define \pvtext \cup \set{\pivotA \spr{i}}$
              \STATE flip $\vps'[i]$
          \ENDIF
        \ELSIF{$\mA \spr{i, j} = 1$}
            \STATE flip $\vps'[i]$
        \ENDIF
    \ENDIF
    \ENDFOR
    \STATE \Return{$\pvtext, \vps', \vsat'$}
  \end{algorithmic}
\end{algorithm}

\begin{algorithm}[tb]
  \caption{$\incensuresatisfaction$ adds a set of pivot rules to ensure that adding rule $i$ as the last free rule to the current prefix satisfies \Axb.}
  \begin{algorithmic}
    \STATE $\pvtext \define \text{an empty set}$
    \FOR{$i=1\ldots\text{rank}(\mA)$}
        \IF{$j = -1$ and $\vb[i] = 1$}
            \STATE $\pvtext \define \pvtext \cup \set{\pivotA \spr{i}}$
            \STATE \Continue
        \ENDIF
        \IF{ $\vsat[i] = 0$}
            \IF{$\pr{\mA\spr{i, j} = 0 \text{ and } \vps\spr{i}\neq\vb\spr{i}}$ \\ $\text{ or } \pr{\mA\spr{i, j} = 1 \text{ and } \vps\spr{i}=\vb\spr{i}}$}

                \STATE $\pvtext \define \pvtext \cup \set{\pivotA \spr{i}}$
            \ENDIF
        \ENDIF
     \ENDFOR
  \STATE \Return{$\pvtext$}
  \end{algorithmic}
\end{algorithm}

\cnote[Han]{the input should be the truth table, not the rules itself. Or we can build the truth table in the algorithm.}

\begin{algorithm}[tb]
  \caption{Incremental branch-and-bound algorithm for enumerating all decision sets whose objective values are at most $\ub$}
  \begin{algorithmic}
    \STATE $\mA, \vb \define \rref \pr{\mA, \vb}$
    \IF{$\Axb$ is unsolvable}
        \STATE exit
    \ENDIF
    \STATE $\solcounter \define 0$
    \STATE $d_{\emptyset} \define \incensuresatisfaction\pr{-1, \vzero, \mA, \vb}$
    \STATE increment $n$ and yield $d_{\emptyset}$ if $R(d_{\emptyset}) < \ub$
    \STATE $d, \vps, \vsat \define \incensurenoviolation\pr{-1, \vzero, \vzero, \mA, \vb}$
    \STATE $\vu \define \lnot \pr{\lor_{j \in d}  \truthtbl\spr{j}}$
    \STATE $Q \define \queue\pr{\spr{\pr{d, b(d), \vu, \vps, \vsat}}}$

    \WHILE{$Q$ not empty and $\solcounter < B$}
        \STATE$\pr{d, b(d), \vu, \vps, \vsat} \define Q.pop()$
        \FOR{$i = \pr{\freeset(d)_{max} + 1}, \ldots, M \text{ and } i \text{ is free}$}
            \STATE \Continue if $\floor{(\ub - b(d)) / \lambda} < 1$ or $b(d') > \ub$
            \STATE $b(d') \define b(d) + \inclb\pr{\vu \land \truthtbl\spr{i}, \vy} + \lambda$
            \IF{$b(d') + \lambda \le \ub$}
                \STATE$\pr{\pvtextone, \vps_q, \vsat_q} \define \incensurenoviolation\pr{i, \vps, \vsat, \mA, \vb}$
                \STATE $d_q \define d \cup \pvtextone \cup \set{i}$
                \STATE $\vv_q \define \vu \land \pr{\lor_{j \in \pr{\pvtextone \cup \set{i}}} \truthtbl\spr{j}}$
                \STATE $b(d_q) \define b(d) + \inclb\pr{\vv_q, \vy} + \pr{\abs{\pvtextone} + 1} \cdot \lambda$
                \STATE $\vw \define \vv_q \lor \pr{\lnot \vu}$
                \IF{$b(d_q) + \txtred{\lambda} \le \ub$}
                    \STATE push $\pr{d_q, b(d_q), \lnot \vw, \vps_q, \vsat_q}$ to $Q$ 
                \ENDIF
            \ENDIF
            \STATE $\pvtexttwo \define \incensuresatisfaction\pr{i, \vps, \vsat, \mA, \vb}$
            \STATE $d_s \define d \cup \pvtexttwo$
            \STATE $\vv_s  \define \vu \land \pr{\lor_{j \in \pr{\pvtexttwo \cup \set{i}}} \truthtbl\spr{j}}$
            \STATE $R(d_s) \define b(d) + \inclb\pr{\vv_s, \vy} + \incobj\pr{\vu, \vv_s, \vy} + \pr{\abs{\pvtexttwo} + 1} \cdot \lambda$
            \STATE increment $\solcounter$ and yield $d_s$ if $R(d_s) \le \ub$
        \ENDFOR
    \ENDWHILE
  \end{algorithmic}
\end{algorithm}




==> archive.tex <==
\section{Preliminaries}
\label{sec:prelim}


\begin{itemize}
\item $S=\set{p_1, \ldots, p_M}$: the set of rule candidates, where we assume a lexicographical order of the candidates, indicated by the subscript index.
\item $d \subseteq \set{1, \ldots, M}$: the indices of rules for a rule set \inote{should elements of $d$ be indices or rules? }
\item if not stated otherwise, we represent $d$ as an ordered list.
\item given two prefixes $d$ and $d'$, we say $d'$ \textit{starts with} $d$ if $d$ is a prefix of $d'$. \inote{should I use decision set instead of prefix?}
\item alternatively, we can represent a rule set $d$ as a binary vector $x_d \in \bindom^{M}$, where $x_d[i] = 1$ if $r_i \in d$ and $x_d[i] = 0$ otherwise.
\item for a given prefix $d$ and a data point, denote $\capt{x, d} = 1$ is at least one rule in $d$ captures $x$ and 0 otherwise.
\item {further for a given rule $p_k \in d$, we define $\capt{x, p_k \mid d} = 1$ if $x$ is captured by $p_k$ but not by rules in $d$ that are ordered before $p_k$ i.e.,
    \[
      \capt{x, p_k \mid d} = \pr{\Land\limits_{p_{k'} \in d \mid k' < k } \lnot\capt{x, p_{k'}}} \land \capt{x, p_k}
    \]
  }
\item for a given rule $p_j \in S$, we denote its \textit{coverage vector} as $\truthtbl\spr{j} \in \bindom^{N}$, where $\truthtbl\spr{j}[i] = \capt{x_i, p_j}$, and $0$ otherwise, for $i = 1, \ldots, N$.
\item $\dmax=\max\set{i \mid i \in d}$: the largest rule index in $d$ if $d \neq \emptyset$, or $\dmax=-1$ if $d = \emptyset$.
\end{itemize}


\cnote[Han]{Perhaps move the definitions of loss and objective to preliminary}

\subsection{Learning objective}

In the sequel, we drop the notations' dependency  on $\pr{\vx, \vy}$ when the context is clear

First we define the objective for a given prefix $d = \pr{p_1, \ldots, p_K}$ as

\begin{equation}
  \label{}
  \obj(d; \lambda) = \loss \pr{d} + \lambda \abs{d}, 
\end{equation}

It consists of the misclassification error $\loss \pr{d}$ , and a regularization term $\lambda \abs{d}$.

The misclassification error term can be decomposed into:

\begin{equation}
  \label{}
  \loss \pr{d} = \lossp \pr{d} + \loss_0 \pr{d}
\end{equation}

where

\begin{equation}
  \label{}
  \lossp \pr{d} = \frac{1}{N} \sum_{n=1}^{N} \sum_{k=1}^{K} \capt{x_n, p_k \mid d} \land \ind{y_n \neq 1}
\end{equation}

\cnote[mc]{Maybe here it should be $ \capt{x_n, d} $ rather than $ \capt{x_n, p_k \mid d}  $ ? }

and

\begin{equation}
  \label{}
  \lossz \pr{d} = \frac{1}{N} \sum_{n=1}^{N} \lnot \capt{x_n, d} \land \ind{y_n = 1}
\end{equation}

Note that $\lossp$ is equivalent to the ratio of false positives while $\lossz$ is the ratio of false negatives.


\subsection{Rashomon set of decision rules}

Given a set of decision rule candidates $\cands$, a objective function $\obj(\cdot; \lambda)$, $\ub \in \real^+$, we define the Rashomon set of $S$ w.r.t. $\ub$ as

\begin{equation}
  \label{}
  \rssverbose = \set{d \subseteq S \mid \obj \pr{d; \lambda} \le \ub}
\end{equation}

When context is clear, we drop the dependency on $\lambda$ and $\ub$, and use $\rssshort$ instead.


\section{Exact counting and uniform sampling of Rashomon decision sets}


\subsection{Problem formulation}
\label{subsec:label}

We consider two related problems about Rashomon decision sets:

\begin{enumerate}
\item counting: calculating $\abs{\rssshort}$.
\item sampling uniformly at random from $\rssshort$.
\end{enumerate}


We address both problems by enumerating all solutions $\rssshort$, which is formalized below:

\begin{problem}[\textbf{Exhaustive enumeration}]
Given a set of decision rule candidates $S$, objective function $\obj$, and $\ub \in \real^+$, enumerate all elements in $\rssverbose$.
\end{problem}


\subsection{A branch-and-bound algorithm}

The proposed branch-and-bound algorithm relies on a few important properties of the objective function, which allows us to prune the search space in an hierarchical way.

We arrive at the property, we eliminate the $\lossz$ term from $\obj$ and define an lower bound of the objective:

\begin{equation}
  \label{}
  \lb \pr{d} = \lossp \pr{d} + \lambda \abs{d}
\end{equation}

Then we have the following bounds:

\begin{theorem}[\textbf{Hierarchical objective lower bound}]
  For any prefix $d \in \spr{M}$, define $d' \in \delta(d)$ to be any prefix that starts with $d$, it follows that $\lb(d) \le \obj(d')$.
  \label{thm:hier-obj-lb}
\end{theorem}
\begin{proof}
  We first prove $\lossp \pr{d} \le  \lossp \pr{d'}$.
  Since $d'$ starts with $d$, we have:
  \begin{align*}
    \lossp (d') & = \frac{1}{N} \sum_{n=1}^{N} \sum_{k=1}^{\abs{d'}} \capt{x_n, p_k \mid d'} \land \ind{y_n \neq 1} \\
                & = \frac{1}{N} \sum_{n=1}^{N} \pr{\sum_{k=1}^{\abs{d}} \capt{x_n, p_k \mid d} \land \ind{y_n \neq 1} + \sum_{k=\abs{d}}^{\abs{d'}} \capt{x_n, p_k \mid d'} \land \ind{y_n \neq 1}  }\\
                &= \lossp (d) +  \frac{1}{N} \sum_{n=1}^{N} \sum_{k=\abs{d}}^{\abs{d'}} \capt{x_n, p_k \mid d'} \land \ind{y_n \neq 1}  \\
                &\ge \lossp (d)\\    
  \end{align*}

  Since $d \subset d'$, $ \abs{d} < \abs{d'}$.
  
  Finally, $\lb(d) = \lossp \pr{d} + \abs{d} \le \lossp \pr{d'} + \abs{d'} + \lossz \pr{d'} = \obj(d')$  
  
\end{proof}

\begin{theorem}[\textbf{Look-ahead bound}]
  For a given prefix $d \in \spr{M}$, if $\lb(d) + \lambda > \ub$, then for any prefix $d'$ that starts with $d$,
  it follows that $\obj(d') > \ub$.
\end{theorem}

\begin{proof}
  Based on the facts that $\lossp(d') \ge \lossp(d)$ and $\abs{d'} \ge \abs{d}$, it follows:
  \begin{align*}
    \obj(d') & = \lossp(d') + \lossz(d') + \lambda \abs{d'} \\
             & \ge \lossp(d) +  \lambda \abs{d} = \lb(d)  \ge \ub \\
  \end{align*}
\end{proof}

\cnote[Han]{TODO: add length bound}
Using the above bounds, we can use the following Algorithm~\ref{alg:noninc-bb} to enumerate the full set of solutions.

\cnote[Han]{use hierarchical objective lower bound to motivate the branch-and-bound algorithm}

\begin{algorithm}[H]
  \KwData{a set of rule candidates $S$, objective upper bound \ub}
  \KwResult{a list of rule sets with objective at most $\ub$}
  $Q \define \queue\pr{\spr{\pr{\emptyset, 0}}}$\;
  \While{$Q$ not empty}{
    $d \define Q.pop()$\;
    \For(\htcp{\textbf{branch}}){$i \in \pr{\dmax + 1}, \ldots, M$}{
      $d' \define d \cup \set{i}$\;
      \If(\htcp{\textbf{hierarchical lower bound}}){$b(d') \le  \ub$}{
        \lIf(\htcp{look-ahead bound}){$\lb(d') + \lambda \le \ub$}{$Q.push\pr{d'}$}
        \lIf{$\obj(d') \le  \ub$}{
          yield $d'$%
        }      
      }            
    }    
  }
  \caption{a branch-and-bound algorithm for enumerating all decision sets whose objective values are at most $\ub$}
  \label{alg:noninc-bb}
\end{algorithm}

\subsection{Incremental computation}

The lower bound and objective function can be incrementally computed, as shown below.

Let $d'$ be a prefix of length starting with $d$ and has exactly one more rule than $d$ as well, i.e., $d' = d \cup \set{p}$, for some $p$.

\begin{align*}
  \label{}
  \lb \pr{d'} &=  \lossp \pr{d'} + \lambda \abs{d'}\\
              &=  \frac{1}{N} \sum_{n=1}^{N} \sum_{k=1}^{\abs{d'}} \capt{x_n, p_k \mid d'} \land \ind{y_n \neq 1} + \lambda \abs{d'}\\
              &=  \frac{1}{N} \sum_{n=1}^{N} \sum_{k=1}^{\abs{d}} \capt{x_n, p_k \mid d'} \land \ind{y_n \neq 1} + \lambda \abs{d} + \lambda + \frac{1}{N} \sum_{n=1}^{N} \capt{x_n, p \mid d'} \land \ind{y_n \neq 1} \\
              &=  \lb \pr{d} + \lambda + \frac{1}{N} \sum_{n=1}^{N} \capt{x_n, p \mid d'} \land \ind{y_n \neq 1} \\
              &=  \lb \pr{d} + \lambda + \frac{1}{N} \sum_{n=1}^{N} \lnot\capt{x_n, d} \land \capt{x_n, p} \land \ind{y_n \neq 1} \\
\end{align*}

Note that the quantity $\lb \pr{d}$ can be cached for incrementally computing $\lb \pr{d'}$.

The objective function can incrementally evaluated based on the lower bound value.

\begin{align*}
  \label{}
  \obj \pr{d'} &= \lossp \pr{d'} + \lossz \pr{d'} + \lambda \abs{d'} \\
               &= \lb \pr{d'} + \lossz \pr{d'} \\
               &= \lb \pr{d'} + \lossz \pr{d'} \\
               &= \lb \pr{d'} + \frac{1}{N} \sum_{n=1}^{N} \lnot \capt{x_n, d'} \land \ind{y_n = 1} \\
               &= \lb \pr{d'} + \frac{1}{N} \sum_{n=1}^{N} \lnot \capt{x_n, d} \land \pr{\lnot \capt{x_n, p}} \land \ind{y_n = 1}
\end{align*}


See Algorithm~\ref{alg:inc-lb-obj} for incremental computation and Algorithm~\ref{alg:inc-bb} for integrating the above computation into the branch and bound algorithm.

\begin{algorithm}[H]
  \Fn{$\inclb\pr{\vv, \vy}$}{
    \tcp{calculates the incremental ratio of false positives}
    \tcp{$\vv$ is the captured vector by a rule in a given context}
    \tcp{$\vy$ is the label vector}
    $n \define \vsum{\vv}$\;
    $\vw \define \vv \land \vy$\;
    $t \define \vsum{\vw}$\;
    \Return{$\pr{n - t} / \len{\vy}$}\;
  }
  \Fn{$\incobj\pr{\vu, \vv, \vy}$}{
    \tcp{calculates the ratio of false negatives}
    \tcp{$\vu$ is the not-captured vector of a given context}
    \tcp{$\vv$ is the captured vector by a rule in the context}
    \tcp{$\vy$ is the label vector}    
    $\vf \define \vu \land \neg \vv$\ratcp{not captured by both }
    $\vg \define \vf \land \vy$\ratcp{false negatives}
    $n_g = \vsum{\vg}$\;
    \Return{$n_g / \len{\vy}$}\;
  }
  \caption{Incremental calculation of lower bound and objective for a rule in the context of a given prefix.}
  \label{alg:inc-lb-obj}
\end{algorithm}


\begin{algorithm}
  \KwData{a set of rule candidates $S$, objective upper bound \ub, regularization parameter $\lambda$, and training data $\pr{\vx, \vy}$}
  \KwResult{a list of rule sets with objective at most $\ub$}
  $Q \define \queue\pr{\spr{\pr{\emptyset, 0}}}$\;
  \While{$Q$ not empty}{
    $ \pr{d, b(d), \vu} \define Q.pop()$\;
    \For(\htcp{branch}){$i \in \pr{\dmax + 1}, \ldots, M$}{
      $d' \define d \cup \set{i}$\;
      $\vv \define \vu \land \truthtbl_i$\;
      $b(d') \define b(d) + \inclb\pr{\vv, \vy}$\;
      \If(\htcp{bound} ){$b(d') \le \ub$}{

        \If{$b(d') + \lambda \le \ub$}{
          $\vu' \define \vu \lor \lnot \truthtbl_i$\;
          $Q.push\pr{\pr{d', b(d'), \vu'}}$\;
        }
        $R(d') \define b(d') + \incobj\pr{\vu, \vv, \vy}$\;
        \lIf{$R(d') \le  \ub$}{
          yield $d'$%
        }
      }        
    }
  }
  \caption{Incremental branch-and-bound algorithm for enumerating all decision sets whose objective values are at most $\ub$}
  \label{alg:inc-bb}
\end{algorithm}



\begin{algorithm2e}
  \KwData{a problem instance of decision set learning $\instance = \pr{\cands, \obj, \ub}$, error tolerance parameter $\epsilon$, confidence parameter $\delta$}
  \KwResult{an estimate of $\abs{\rss}$}
  $\budget \define 1+ 9.84 \pr{1 + \frac{\tol}{1+\tol}}^2$\;
  $\solset \define \algbs \pr{\instance, \budget}$\;
  \lIf{$\abs{\solset} < \budget$}{\Return{$\abs{\solset}$}}
  $t \define \ceil{17 \log_2 \pr{3 / \confi}}$\;
  $\ncells  \define 2;\ C \define \spr{};\ i \define 0$\;
  \While{$i < t$}{
    increment $i$\;
    $\pr{\ncells, \solcount} \define \algacc \pr{\instance, \budget, \ncells}$\;
    \lIf{$\ncells \neq \txtnull$}{add $\solcount$ to $C$}
  }
  \Return{$\text{median}\pr{C}$}
  \caption{\algac\xspace takes in an instance of decision set learning and outputs an estimate of the Rashomon set size}
  \label{alg:approxcount}
\end{algorithm2e}

\begin{algorithm}[H]
  \KwData{a problem instance of decision set learning $\instance = \pr{\cands, \obj, \ub}$, budget $\budget \in \real^+$, and the number of cells computed from previous run $\prevncells$}
  \KwResult{an estimate of $\abs{\rss}$}
  Draw $\mA$ from $\bindom^{\abs{\cands} \times \pr{\abs{\cands} - 1}}$ uniformly at random\;
  Draw $\vb$ from $\bindom^{\abs{\cands} - 1}$ uniformly at random\;
  $\solset \define \algbs \pr{\instance, \Axb, \budget, \prevncells}$\;
  \lIf{$\abs{\sols} \ge \budget$}{\Return{\txtnull}}
  $\pr{m, c} \define \algls \pr{\instance, \Axb, \budget, m}$\;
  \Return{$\pr{2^m, c \times 2^m}$}
  \caption{\algacc\xspace takes in one instance of decision set learning and outputs the number of cells and an estimate of $\abs{\rss}$.
  }
\end{algorithm}

\begin{algorithm}[H]
  \KwData{a problem instance $\instance = \pr{\cands, \obj, \ub}$, budget $\budget \in \real^+$, parity constraint system $\Axb$, and the initial number of constraints $\prevm$}
  \KwResult{estimated number of constraints to use $m$ and the corresponding solution size $\abs{\rss \cap \mA_{1:m} x = \vb_{1:m}}$}
  $\loidx \define 0;\ \hiidx \define \abs{\cands} - 1; \ m \define \prevncells$\;
  $\bigcell[0] \define 1;\ \bigcell[\abs{\cands} - 1] \define 0; \ \bigcell[i] \define \nullresult\; \forall i \not\in \set{0, \abs{\cands} - 1}$\;
  \While{\true}{
    $\solset \define \algbs \pr{\instance, \mA_{:m} x = \vb_{:m}, \budget}$\;
    \eIf{$\abs{\solset} \ge \budget$}{
      \lIf{$\bigcell \pr{m+1} = 0$}{\Return{$m+1$}}
      $\bigcell[i] \define 1\; \forall i \in \set{1, \ldots, m}$\;
      $\loidx \define m$\;
      \lIf{$|m - \prevm| < 3$}{
        $m \define m+1$
      }
      \lElseIf{$2 \cdot m < \abs{\cands}$}{
        $m \define 2 \cdot m$
      }
      \lElse{
        $m \define \pr{\hiidx + m} / 2$
      }
    }{
      \lIf{$\bigcell[m-1] = 1$}{\Return{$m$}}
      $\bigcell \spr{i} \define 0\; \forall i \in \set{m, \ldots, \abs{\cands}}$\;
      $\hiidx \define m$\;
      \lIf{$|m - \prevm| < 3$}{
        $m \define m -1$
      }
      \lElse{
        $m \define (m + \loidx) / 2$
      }
    }
  }
  \caption{\algls\xspace finds the number of constraints under which the number of feasible solutions is below but closest to $\budget$.}
  \label{alg:logsearch}
\end{algorithm}

\begin{algorithm}[H]
  \KwData{a problem instance $\instance = \pr{\cands, \obj, \ub}$ and tolerance parameter $\tol$}
  \KwResult{a decision set drawn from $\rss$}
  \caption{\algsample draws a random sample from $\rss$ almost uniformly at random}
  $\pr{\kappa, \unigenpivot} \define \algkappapivot(\tol)$\;
  $\hibudget \define 1 + (1 + \kappa) \unigenpivot$\;
  $\lobudget \define \frac{1}{1 + \kappa} \unigenpivot$\;
  $\solset  \define \algbs(\instance, \hibudget)$\;
  \lIf{$\abs{\solset} \le \lobudget$}{
    \Return{$s \sim \unirandom \pr{\solset}$}
  }
  \Else{
    $\solcount \define \algac(\instance, 0.8, 0.8)$\;
    $q \define \ceil{\log\solcount + \log 1.8 - \log \unigenpivot}$\;
    $i \define q - 4$\;
    $\mA \sim \unirandom \pr{\bindom^{\abs{\cands} \times \pr{\abs{\cands} - 1}}}$ and $\vb \sim \unirandom \pr{\bindom^{\abs{\cands} - 1}}$\;
    \Repeat{$\lobudget \le \abs{\solset} \le \hibudget$ or $i = q$}{
      $i \define i + 1$\;
      $\solset \define \algbs \pr{\instance, \mA_{:i} x = \vb_{:i}, \hibudget}$\;
    }
    \lIf{$ \lobudget \le \abs{\solset} \le  \hibudget$}{\Return{$\unirandom \pr{\solset}$}}
    \lElse{\Return $\nullresult$}
  }

\end{algorithm}

\begin{algorithm}[H]
  \KwData{a set of rules $S$, objective upper bound \ub, regularization parameter $\lambda$, training data $\pr{\vx, \vy}$, parity constraint system $\Axb$, and the maximum number of solutions $B$ to find}
  \KwResult{a list of rule sets with objective at most $\ub$}
  $\mA, \vb \define \rref \pr{\mA, \vb}$\;
  \lIf{$\Axb$ is unsolvable}{exit}
  $\solcounter \define 0$\;
  \tcp{the case that no free rules are added}  
  $d_s \define \ensuresatisfaction\pr{\emptyset, \mA, \vb}$\;
  \lIf{$R(d_s) \le \ub$}{increment $n$ and yield $d_s$}
  $d_q \define \ensurenoviolation\pr{\emptyset, \mA, \vb}$\;
  $Q \define \queue\pr{\pr{d_q}}$\;
  \While{$Q$ is not empty and $\solcounter < B$}{
    $d \define Q.pop()$\;
    \For{$j = \pr{\freeset(d)_{max} + 1}, \ldots, M \text{ and } i \text{ is free}$}{
      $d' \define d \cup \set{j}$\;
      \If(\htcp{hierarchical lower bound}){$b(d') \le \ub$}{        
        $\pvtextone \define \ensurenoviolation\pr{d', \mA, \vb}$\;
        \lIf{$b(d' \cup \pvtextone) < \ub$}{$Q.\text{push}(d')$} 
        $\pvtexttwo \define \ensuresatisfaction\pr{d', \mA, \vb}$\;
        $d_s \define d' \cup \pvtexttwo$\;
        \lIf{$R(d_s) \le \ub$}{
          increment $\solcounter$ and yield $d_s$
        }          
      }
    }
  }
  \caption{Naive branch and bound to solve Problem~\ref{prob:budgeted-enum}.
    The incremental calculation of objective lower bound and objective value is omitted for brevity.}
  \label{alg:noninc-cbb}
\end{algorithm}

\begin{algorithm}[H]
  \caption{
    $\ensurenoviolation$ extends a prefix $d$ by a set of necessary pivot rules such that the new prefix is minimally non-violating
  }
  \label{alg:ensure-non-vio}
  \begin{algorithmic}

  \end{algorithmic}
  \Fn{$\ensurenoviolation\pr{d, \mA, \vb}$}{
    $\vr = \vb - \mA \cdot \xd$\;
    $\pvtext \define \emptyset$\;    
    \For{ $i = 1, \ldots, \rank\pr{\mA}$ }{
      \lIf{$\vr[i] = 1$ and $\dmax \ge \btbl[i]$}{
        $\pvtext \define \pvtext \cup \pivotA[i]$
      }
    }
    \Return{$\pvtext$}
  }
\end{algorithm}


==> case_study.tex <==

As a simple case study, we show how the proposed methods allow to efficiently estimate feature (or variable) importance. 
In particular, the goal of the case study is to demonstrate that
reliable estimates of feature importance can be derived from samples of rule sets in the Rashomon set. 
The main results are summarized in Section~\ref{subsec:compas-case-study}. 
In this section, we provide additional details. 



Different measures of feature importance have been proposed~\cite{saarela2021comparison}. 
Recent work focuses on \emph{model reliance}~\cite{fisher2019all,xin2022exploring}. 
Model reliance captures the extent to which a model relies on a given feature to achieve
its predictive performance. 
For our purposes, given rule set $\rs$ and feature $v$, we define model reliance as follows: 
\begin{equation}\label{eq:modelReliance}
	MR(\rs, v) = \frac{\obj(\rs; v', \lambda)}{\obj(\rs;  v, \lambda)},
\end{equation}

where $\obj(\rs; v, \lambda)$ is the objective achieved by $\rs$ in the original dataset, and $\obj(\rs;  v', \lambda)$ is identical to $\obj(\rs; v, \lambda)$ except that $v$ is replaced by its uninformative counterpart $v'$.
Feature $v'$ is obtained by swapping the first and second halves of the feature values of $v$, thereby retaining the marginal distribution of $v$, while destroying its predictive power. 
This measure is similar to the \emph{model reliance} measure used by~\citet{xin2022exploring}. 


Model reliance evaluates how important a variable is for a given rule set. In particular, the higher model reliance, the more important feature $v$. 
If we have a single rule set $\rs$, we would simply estimate the importance of feature $v$ by $MR(\rs, v)$. 
However, if we have access to the Rashomon set of all near-optimal rule sets, it is more informative to investigate the variation of $MR(\rs, v)$ across rule sets $\rs$ in the Rashomon set. 
Hence, we compute $MCR^-(v)$ and $MCR^+(v)$, the minimum and maximum model reliance for variable $v$ across rule sets in the Rashomon set. %

In Figure~\ref{fig:compas-case-study} (Section~\ref{subsec:compas-case-study}), we compare  $MCR^-(v)$ and $MCR^+(v)$ computed in the entire Rashomon set and in samples or rule sets drawn from the Rashomon set by \algsample, and we conclude that the sample estimates are consistently close to the measures computed in the entire Rashomon set, suggesting that exhaustive enumeration may be redundant when the goal is to investigate feature importance. 




In addition, while model reliance is an adequate measure of the importance of features in the context of a given rule set, $MCR^-(v)$ and $MCR^+(v)$ fail to capture the idea that some features are more frequent than others in the Rashomon set. 
Inutitively, at parity model reliance, the more frequent a feature is in the Rashomon set, the more important. 
Hence, to provide a more complete assessment of feature importance across the Rashomon set, Figure~\ref{fig:casestudy} shows the proportion of rule sets including a given variable in the entire Rashomon set or in a sample of $400$ rule sets obtained using \algsample. 
The reported sample estimates are obtained as averages over $10$ repetitions of the sampling process. 
The relative frequency of the features estimated in the sample and in the entire Rashomon set are remarkably similar, corroborating the findings presented in Section~\ref{subsec:compas-case-study} with respect to model reliance.


\begin{figure*}[t!]
	\centering
	\begin{tabular}{cc}
		\includegraphics[width=0.6\textwidth,height=0.2\textheight,keepaspectratio]{plots/compas_variable_importance_freqs_full_rashomon_set_10_reps.pdf} & 
		\includegraphics[width=0.6\textwidth,height=0.2\textheight,keepaspectratio]{plots/compas_variable_importance_freqs_400_samples_10_reps.pdf} \\
	\end{tabular}
	\caption{\label{fig:casestudy} 
          Relative frequencies of features in the Rashomon set (left) and associated sample estimates (right). 
	}
      \end{figure*}


Finally, we mention that the results do not corresponds exactly to the similar results presented by~\citet{xin2022exploring} because we consider a different class of models and a different loss. However, there are interesting commonalities. For instance, the variable $Prior>3$ has the highest  $MCR^+(v)$ in both studies.



==> case_study_fairness.tex <==




\begin{figure}[t]
  \centering
  \includegraphics[width=0.35\textwidth,height=0.05\textheight,keepaspectratio]{plots/legend_fairness.pdf}
  \includegraphics[width=0.475\textwidth]{plots/boxplot_fairness_test_set_loss.pdf}
  \caption{
    Objective $\obj$ on the test set 
    obtained by the optimal fair rule set found in the train set with respect to different fairness measures. 
    The fairness-constrained optimal objective value is reported 
    for the rule sets 
    of the entire Rashomon set ($100\%$) as well as for samples of increasing size ($10\%$, $20\%$ and  $40\%$).  }
  \label{fig:fairness_2}
\end{figure}


The Rashomon set offers a novel perspective on fairness of machine learning models. 
Although all models in the Rashomon set achieve near-optimal predictive performance, they may exhibit different fairness characteristics.
The Rashomon set allows to %
identify the range of predictive bias produced by the models %
 and to search for models that are both accurate and fair.


We carry out a case study focusing on the \compas dataset,
which has fueled intense debate and research in fair machine learning~\cite{rudin2022interpretable,aivodji2019learning},
and fairness constraints are specified with respect to the \emph{sex} attribute, which partitions the dataset into two groups, \emph{males} (M) and \emph{females} (F).

A concise summary of the case study is given in Section~\ref{sec:fairness_main}. Here, we discuss the details and summarize the key findings. 

First, we introduce the considered measures of fairness. 

\para{Fairness measures.}
Let  $\hat{y}=1$ denote the event that the data record $\vx$ is predicted as positive (i.e. $\capt{\vx, \rs}$).
Moreover, let $x_s$ denote the sex of data record $\vx$. 
We consider 
the following fairness measures~\cite{aivodji2019learning}. 

\begin{itemize}
\item {\emph{Statistical parity} measures the absolute difference of rate of positive predictions between the groups:
    \[
          \abs{\proba{\hat{y}=1|x_s=\text{F}} - \proba{\hat{y}=1|x_s=\text{M}}}.
    \]
}
\item {\emph{Predictive parity} measures the absolute difference of precision between  the groups:
  \[
    \abs{\proba{y=1|\hat{y}=1, x_s=\text{F}} - \proba{y=1|\hat{y}=1, x_s=\text{M}}}.
  \]
}
\item {\emph{Predictive equality} measures the absolute difference of false positive rate between the groups:
    \[
      \abs{\proba{\hat{y}=1| y=0, x_s=\text{F}}- \proba{\hat{y}=1| y=0, x_s=\text{M}}}.
    \]

}	
\item {\emph{Equal opportunity} measures the absolute difference of true positive rate between the groups:
    \[
      \abs{\proba{\hat{y}=1| y=1, x_s=\text{F}} - \proba{\hat{y}=1| y=1, x_s=\text{M}}}.
    \]
}	
\end{itemize}

For all four measures, the larger the value, the more unfair the model is.

\para{Investigating fairness measures by sampling.}
Figure~\ref{fig:fairness_1} in Section~\ref{sec:fairness_main} shows the distribution of the above fairness measures in the entire Rashomon set and in samples of increasing size. 
For each measure, we show the range (minimum and maximum), the interquartile range (first and third quartiles) and the median. 
All such statistics describing the distributions of the fairness measures of interest in the samples of rule sets are obtained as average over $10$ repetitions of the random sampling process.


The Rashomon set consists of $|\rssshort|=1409$ rule sets and we use \algsample to draw samples of sizes $10\%$, $20\%$ and $40\%$ of $|\rssshort|$. 


\para{Finding accurate-yet-fair models by sampling.}
To demonstrate that %
the proposed sampling strategy can be used to find an accurate model while satisfying particular fairness constraints,
we set up a simple two-step experiment.  

\newcommand{\fairmeasure}{\ensuremath{M_{fair}}}
First, given a sample of rule sets from the Rashomon set, we consider any of the four fairness measures described above, say $\fairmeasure$,
and we exclude all models with value of $\fairmeasure$ beyond the first quartile of the distribution of $\fairmeasure$ in the entire Rashomon set. 


The remaining models are referred to %
as fair models (with respect to the chosen $\fairmeasure$). 
Second, among the remaining (fair) models, we pick the model $\rs^*$ which minimizes the objective $\obj$. %


Figure~\ref{fig:fairness_2} reports the value of $\obj$ in the test set for the chosen rule set $m^*$
in the entire Rashomon set and in samples of rule sets of increasing size.  
Again, the Rashomon set consists of $|\rssshort|=1,409$ rule sets and we draw samples of sizes $10\%$, $20\%$ and $40\%$ of $|\rssshort|$ using \algsample. 
The reported losses are obtained as average over $10$ repetitions of the sampling process. 
The performance of the optimal \emph{fair} rule set chosen from the samples is not far from the performance of the optimal \emph{fair} rule set chosen in the entire $\rssshort$, and the gap between the performance of the optimal \emph{fair} rule set in the entire Rashomon set and in samples drawn from it quickly shrinks as the sample size increases. 
In the case of statistical parity, no significant difference is observed across different sample sizes, suggesting that even the smallest sample in enough to find a  rule set which is fair with respect to statistical parity and exhibits predictive performance indistinguishable from the predictive performance of the fair rule set that would be chosen in the entire Rashomon set. 

Thus, in view of the results reported in this section, we conclude that exhaustive enumeration of the Rashomon set may be redundant when the goal is to investigate fairness or find a model that is both accurate and fair. A representative sample may suffice. 




==> diagram_sts.tex <==
To facilitate understanding, Figure~\ref{fig:diagramsts} provides a graphical representation of the partial exploration of the search tree of all rule sets performed by \bbSTS. 
As explained in Section~\ref{sec:tree-sampler}, the exploration of the search tree starts from the root, indicated by a diamond in Figure~\ref{fig:diagramsts}, which represents  the empty rule set $\emptyset$. 
At the $i$-th iteration, \bbSTS subsamples without replacement a number of partial solutions $S \in P_{i-1}$ at depth $i-1$, which are subsets of the first $(i-1) \cdot l$ rules, for some input parameter $l$. Such partial solutions are also referred to as partial solutions of level $(i-1) \cdot l$. 
In Figure~\ref{fig:diagramsts}, the  sampled partial solutions are highlighted in red. 
Then, for each sampled partial solution $S$, \bbSTS carries out \bb-like search to find all larger partial solutions $\{S'\}_i^S$ at depth $i$ (highlighted in blue in Figure~\ref{fig:diagramsts}) that are subsets of the first $i \cdot l$ rules (i.e., they are of level $i \cdot l$) and that start with $S$. 
\bbSTS repeats this procedure until, upon reaching the leaves of the search tree, partial solutions of level $M$ are generated. Partial solutions of level $M$ are such that all rules in \candrules have been considered for inclusion and, provided that they belong to the Rashomon set, are output as near-uniform samples.

\begin{figure*}
\centering
 \scalebox{1}{
\begin{tikzpicture}[root/.style={draw,diamond, minimum size=1mm},
branch/.style={draw,rectangle},
leaf/.style={draw,circle, minimum size=1mm},
level 1/.style={sibling distance=8.5em, level distance=5.5em},
level 2/.style={sibling distance=2.5em},
level 3/.style={sibling distance=2em,},
edge from parent/.style={draw, shorten >=18pt}]
\node [root] (root) { $\emptyset$ }
child { node[branch, circle,minimum size=7mm] (child1) {} %
}
child { node[branch, circle, red, line width=1.2pt,  minimum size=7mm]  (child2) {} %
	child { node[leaf, blue, line width=1.1pt,minimum size=7mm]  (leaf4) {} }
	child { node[leaf, blue, line width=1.1pt,minimum size=7mm]  (leaf5) {} }
	child { node[leaf, blue, line width=1.1pt,minimum size=7mm]  (leaf6) {} }
}
child { node[branch, circle, red, line width=1.2pt, minimum size=7mm]  (child3) {\ensuremath{S}} %
	child { node[leaf, blue, line width=1.1pt,minimum size=7mm] (leaf7) {} }
	child { node[leaf, blue, line width=1.1pt,minimum size=7mm] (leaf8) {} }
	child { node[leaf, blue, line width=1.1pt,minimum size=7mm] (leaf9) {} }
};


\node[right=1.5em of $(child3)!0.5!(child3)$] {depth $i-1$};
\node[right=0.5em of leaf9] {depth $i$};
\node[right=0.25em of root] {depth $0$};

\node[left=10em of $(child1)!0.5!(child3)$] (a1) {level $(i-1) \cdot l $};




\node[left=10em of leaf4]{level $i \cdot l$};;
\node[left=0.25em of root] {level $0$};


\node[above=0.5em of child2] {$\dots$};

\draw (child3) -- (leaf9);
\draw (child3) -- (leaf8);
\draw (child3) -- (leaf7);


\draw (child2) -- (leaf4);
\draw (child2) -- (leaf5);
\draw (child2) -- (leaf6);



\node[fit=(leaf7) (leaf9), draw, inner sep=2pt, thick] {  };
\node[below left=0.5em and -0.1 of leaf8] {$ \{ \ensuremath{S}' \}_i^\ensuremath{S} $}; 

\node[fit=(child1) (child3), draw, inner sep=2pt, thick] {  };
\node[below =0.25em of child1] {$ P_{i-1} $}; 

\node[above right=2em and -3em of child3] (S2) {$ {\textcolor{red}{S}} \subseteq \{ r_1, r_2,\dots r_{(i-1) \cdot l} \}$};
\draw[->, shorten >=1em] (S2) -- (child3);






\node[below left=5.5em and 1.5em of leaf4, leaf, black,minimum size=7mm](leaf11) {};

\node[above right=2em and 0.25em of leaf11,opacity=0] (help11) {};
\draw[] (leaf11) -- (help11);


\node[below left=5.5em and 1.5em of leaf5, leaf, black,minimum size=7mm] (leaf12) {};

\node[above=1.6em of leaf12,opacity=0] (help12) {};
\draw[] (leaf12) -- (help12);

\node[below left=5.5em and 1.5em of leaf6, leaf, black,minimum size=7mm] (leaf13) {};

\node[above left=2em and 0.25em of leaf13,opacity=0] (help13) {};
\draw[] (leaf13) -- (help13);


\node[below left=5.5em and 1.2em of leaf7, leaf, black,minimum size=7mm] (leaf14) {};

\node[above right=2em and 0.25em of leaf14,opacity=0] (help14) {};
\draw[] (leaf14) -- (help14);


\node[below left=5.5em and 1.2em of leaf8, leaf, black,minimum size=7mm] (leaf15) {};

\node[above=1.6em of leaf15,opacity=0] (help15) {};
\draw[] (leaf15) -- (help15);

\node[below left=5.5em and 1.2em of leaf9, leaf, black,minimum size=7mm] (leaf16) {};

\node[above left=2em and 0.25em of leaf16,opacity=0] (help16) {};
\draw[] (leaf16) -- (help16);


\node[below right=5.5em and 4.5em of leaf7, leaf, black,minimum size=7mm] (leaf17) {};

\node[above right=2em and 0.25em of leaf17,opacity=0] (help17) {};
\draw[] (leaf17) -- (help17);


\node[below right=5.5em and 4.5em of leaf8, leaf, black,minimum size=7mm] (leaf18) {};

\node[above=1.6em of leaf18,opacity=0] (help18) {};
\draw[] (leaf18) -- (help18);

\node[above=0.05em of help18] {$\dots$};

\node[above=0.05em of help15] {$\dots$};

\node[above=0.05em of help12] {$\dots$};

\node[below right=5.5em and 4.5em of leaf9, leaf, black,minimum size=7mm] (leaf19) {};


\node[above left=2em and 0.25em of leaf19,opacity=0] (help19) {};
\draw[] (leaf19) -- (help19);


\node[right=0.5em of leaf19] {depth $\lceil \frac{M}{l} \rceil$};

\node[left=10em of leaf11]{level $M$};;


\end{tikzpicture}
}
\caption{Graphical representation of the search carried out by the \bbSTS algorithm. }
\label{fig:diagramsts}
\end{figure*}


==> efficacy_optimzation.tex <==

We study how various optimization techniques affect the running time of \bb.
To this aim, 
we remove each of the three bounds from the full algorithm and measure the corresponding execution information, such as running time, number of lower bound (and objective) evaluations, etc. We consider the \compas dataset, set $\ub=0.25$ and $\lambda=0.05$. 
Results are summarized in Table~\ref{tab:bounds}. 
\inote{This can be moved in its own section in the appendix.}
\begin{center}
	\begin{table}
		\caption{\label{tab:bounds}Effect of removing each pruning bound from Algorithm~\ref{alg:noninc-bb}.}
		\begin{tabular}{l|rrrrr}
			& time (s) & $\lb$ eval. & $\obj$ eval. & $Q$ insert.\\
			\hline
			full & 10.23 & 1.3e+6 & 7.5e+5 &  1.2e+5\\
			\hline
			w/o length & +65\% & +101\% & +58\% & +000\%\\
			w/o look-ahead & +90\% & +000\% & +00\% &  +544\%\\
			w/o hierarchical  & +7\% & +000\% & +76\% & +000\%\\
		\end{tabular}
	\end{table}
\end{center}  


==> experiment_by_rules.tex <==
 
The parameter \ub is the parameter that affects the most the runtime of the proposed algorithms, since, when $\ub$ is increased even slightly, the size of the Rashomon set grows exponentially fast. 
The number $M$ of pre-mined rules which are input to \bb, \bbSTS and \algac also affects the size of the Rashomon set and hence the computational burden associated with the proposed algorithms. 
Thus, we also carry out experiments to evaluate the impact of the number $M$ of input rules on \bb, \bbSTS and \algac. 

We vary the number of input rules $M$ in $(30,50,70,90,110)$, with $\lambda=0.1$ and upper bound \ub fixed to $0.7$, $1.05$, $1.2$ and $1.0$ for \compas, \mush, \voting and \credit, respectively.  
We always consider the first $M$ rules with the highest number of captured data records. 





The results of the experiments, summarized in Figure~\ref{fig:runtime_and_counts_by_number_of_rules},   %
highlight a fundamental observation. When the upper bound \ub is small enough, \bb is often faster than \algac, even when the number of input rules $M$ grows. 
When the number of rules is increased from $M$ to $M'$, additional $M' - M$ rules are added which capture less data records than the first $M$ rules. 
\bb is effective in quickly eliminating large portions of the search space associated with rules of limited support. 
Hence, when the upper bound \ub is small enough to guarantee that \bb scales gracefully, \bb should be preferred over \algac. 
Instead, as shown in Section~\ref{sec:experiment_results}, as the upper bound \ub increases, \algac scales drastically better than \bb. 
Finally, \bbSTS is always considerably faster than both \bb and \algac as either \nrules or \ub increases, and it is therefore the preferred algorithm when scalability is a primary concern and a significant degree of approximation in the counts can be tolerated. 






\begin{figure*}[t]
	\centering
	\includegraphics[width=0.35\textwidth,height=0.05\textheight,keepaspectratio]{plots/legend_main_plot.pdf}
	\begin{tabular}{cccc}
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/runtime_by_rules_compas__larger_range_07_110.pdf} &
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/runtime_by_rules_mushrooms__larger_range_105.pdf} &
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/runtime_by_number_of_rules_voting_larger_range_110_02.pdf} &
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/runtime_by_number_of_rules_credit_larger_range_110_01.pdf} \\
		\compas &
		\mush &
		\voting &
		\credit \\
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/counts_by_number_of_rules_compas_larger_range_log_0_7_110.pdf} &
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/counts_by_number_of_rules_mushrooms1_05_log.pdf} &
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/counts_by_number_of_rules_votinglarger_range_log_110_02.pdf} &
		\includegraphics[width=0.22\textwidth,height=0.2\textheight,keepaspectratio]{plots/counts_by_number_of_rules_creditlarger_range_log_110_1_0.pdf} \\
		\compas &
		\mush &
		\voting &
		\credit \\
	\end{tabular}
	\caption{\label{fig:runtime_and_counts_by_number_of_rules} Top: runtime (seconds) by number of rules. Bottom: counts by number of rules (on log scale). }
\end{figure*}





==> illustrations/cbb.tex <==
\begin{figure}[h]
  \begin{tabular}{cc}
    \begin{tikzpicture}[
      every node/.style={%
      },
      level distance=10mm,
      level 1/.style={sibling distance=6.5mm},
      level 2/.style={sibling distance=4mm}
      ]
      \node [anchor=north west] {$\emptyset$}
      child {node {$2^*$}
        child {node[xshift=-4mm] {$6^* (0)$}}  %
        child {node[xshift=4mm] {$7^*$}}
      }
      child {node {$3$}}
      child {node {$5$}}
      child {node {$7^*$}}
      ;
    \end{tikzpicture} & \begin{tikzpicture}[
      every node/.style={%
      },
      level distance=10mm,
      level 1/.style={sibling distance=6.5mm},
      level 2/.style={sibling distance=4mm}
      ]                      
      \node [anchor=north west] {$\emptyset$} 
      child {node {$1$}}
      child {node {$2^*$}
        child {node {$6^*$}}
        child {node {$7^*$}}
      }
      child {node {$3$}}
      child {node {$5$}}
      child {node {$6^*$}
        child {node {$7^*$}}
      }
      child {node {$7^*$}};

    \end{tikzpicture}  \\
    \scalebox{0.8}{
    $\begin{bmatrix}
       1 & 0 & 0 & 1 & 1 \\
       0 & 1 & 0 & 0 & 0
     \end{bmatrix}
    x
    =
    \begin{bmatrix}
      0 \\
      0 \\
    \end{bmatrix}$ }&
                      \scalebox{0.8}{
                      $\begin{bmatrix}
                         1 & 0 & 0 & 0 & 1 \\
                       \end{bmatrix}
                      x
                      =
                      \begin{bmatrix}
                        0 \\
                      \end{bmatrix}$ }\\        
    $(a)$ estimated count $4 \times 2^2$ & $(b)$ estimated count $6 \times 2^1$ \\
    \multicolumn{2}{c}{
    \begin{tikzpicture}[
      every node/.style={%
      },
      level distance=10mm,
      level 1/.style={sibling distance=6mm},
      level 2/.style={sibling distance=4mm}
      ]
      \node at (1.5, 2) [anchor=north west] {$\emptyset$} 
      child {node {$0^*$}
        child {node {$2^*$}
          child {node {$6^*$}}
        }
      }
      child {node {$1$}}
      child {node {$2^*$}
        child {node {$4^*$}}
        child {node {$6^*$}}
        child {node {$7^*$}}
      }
      child {node {$3$}}
      child {node {$4^*$}
        child {node {$6^*$}}
        child {node {$7^*$}}
      }
      child {node {$5$}}
      child {node {$6^*$}
        child {node {$7^*$}}
      }
      child {node {$7^*$}}
      ;
    \end{tikzpicture}     
    } \\
    \multicolumn{2}{c}{
    $(c)$  true count = 13
    }                      
  \end{tabular}
  \caption{Illustration of the approximate counting algorithm on a toy dataset with 8 rules.
    Exact enumeration in random cells are repeated sufficiently enough times and the median is shown.    
    The search trees in two random cells ($(a)$ and $(b)$) are shown for illustration purpose ($(c)$ shows the search tree in the whole solution space).
    The node labels represent the index of the rule being checked.
    Nodes corresponding to feasible solutions are annotated with $*$.
    For instance in $(a)$, leaf node labeled with $7^*$ corresponds to the solution of $\set{2, 7}$.
    The number in the parenthesis (e.g., $(0)$ in $(a)$) represents the index of rules that must be selected to satisfy the $\Axb$ (more details later).
  }
  \label{fig:cbb}
\end{figure}

